Model-based Preference Optimization in Abstractive Summarization without Human Feedback

In abstractive summarization, the challenge of producing concise and accurate summaries arises from the vast amount of information contained in the source document. Consequently, although Large Language Models (LLMs) can generate fluent text, they often introduce inaccuracies by hallucinating content not found in the original source. While supervised fine-tuning methods that maximize likelihood contribute to this issue, they do not consistently enhance the faithfulness of the summaries. Preference-based optimization methods, such as Direct Preference Optimization (DPO), can further refine the model to align with human preferences. However, these methods still heavily depend on costly human feedback. In this work, we introduce a novel and straightforward approach called Model-based Preference Optimization (MPO) to fine-tune LLMs for improved summarization abilities without any human feedback. By leveraging the model's inherent summarization capabilities, we create a preference dataset that is fully generated by the model using different decoding strategies. Our experiments on standard summarization datasets and various metrics demonstrate that our proposed MPO significantly enhances the quality of generated summaries without relying on human feedback.

==> scripts/1_intro_original.tex <==

\section{Introduction}
\label{sec:intro}



Large Language Models (LLMs; \citet{gpt3}, \citet{llama1}, \citet{mistral}) have shown remarkable capabilities in generating fluent and plausible text. However, despite these advancements, LLMs often produce summaries that are plausible yet contain incorrect or contradictory information, a phenomenon referred to as \textit{hallucination} \cite{maynez-etal-2020-faithfulness}. This issue stems from the training of LLMs using maximum likelihood, the most common objective for pre-training language models~\cite{king2022dont, tian2024finetuning}.
Naively fine-tuning with faithfulness-aware objectives, which seems straightforward, can fail to ensure factual accuracy~\cite{wan2022factpegasus} and may diminish the model's ability to produce useful summaries~\cite{chae2024mitigating}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/radar_chart.png}
    \caption{\textbf{Comparison with human preference optimized models.} This is the result of the GPT-J model on the TL;DR dataset. The method FAPO, which uses the model-generated results to build a preference dataset for preference optimization, proves to be more effective than PPO (w/ human preferences) and DPO (w/ human preferences), both of which use human preference datasets for preference optimization.}
    \label{fig:radar_chart}
\end{figure}


In response, \citet{tian2024finetuning} have suggested using reinforcement learning-based objectives~\cite{dpo}, which circumvent the limitations of traditional pre-training methods by selecting reward functions that penalize factually incorrect statements. However, the process of acquiring human labels for factuality to optimize preferences is both time-consuming and costly. Moreover, \citet{hosking2024human} emphasized that human feedback has bias and under-represent in terms of factuality. 
Our empirical results also showed that utilizing human preference data as a training objective do not necessarily enhance factuality. 
Furthermore, hiring human annotators is prohibitively expensive.  According to \citet{min2023factscore}, professional fact-checkers required approximately 9 minutes to verify a single model-generated biography of a well-known figure, costing about \$2,000 to annotate 505 biographies.



In this study, we propose a method for constructing a preference dataset that leverages the model's internal awareness without relying on human feedback. Rather than employing a typical human preference dataset for optimization, we utilized the outputs generated by the language model itself~\cite{kadavath2022language, tian-etal-2023-just}. Specifically, we exploit the differences between deterministic and stochastic decoding in abstractive summarization~\cite{welleck-etal-2020-consistency}. We used outputs from beam search decoding as the preferred pairs and outputs from random sampling at a set temperature as the rejected pairs to construct our preference dataset.

Numerous studies~\cite{yang-etal-2018-breaking, welleck-etal-2020-consistency, Holtzman2020The} indicate that deterministic decoding, compared to stochastic decoding, exhibits less surprising characteristics, which may aid in generating summaries that are more faithful to the input document. \citet{wan-etal-2023-faithful-generation} find a consistent trend where beam search provides the most faithful summaries, while the randomness introduced by sampling diminishes faithfulness.



For our experiments, we used well-known datasets such as Reddit TL;DR and XSUM \cite{tldr, xsum}, and models including GPT-J, LLaMA2-7B, and Mistral-7B \cite{gpt3, touvron2023llama, mistral}. To evaluate summarization performance, we employed six different metrics as in \citet{chae2024mitigating}. As a result, faithfulness-aware preference optimization with self-feedback showed overall robust performance on evaluation metrics. 




==> tables/main.tex <==
\begin{table*}[t!]
\centering
\resizebox{1\textwidth}{!}{%
% \begin{tabular}{c|l|llllllllllll}
\begin{tabular}{c|c|l|cccccccccc}
\noalign{\hrule height 1pt}
\multicolumn{2}{c}{}        &                                   & \multicolumn{2}{c}{\textbf{AlignScore (\uparrow)}}                        & \multicolumn{2}{c}{\textbf{FactCC (\uparrow)}}                            & \multicolumn{2}{c}{\textbf{BARTScore (\uparrow)}}                         & \multicolumn{2}{c}{\textbf{BS-FACT (\uparrow)}}                           & \multicolumn{2}{c}{\textbf{ROUGE-L(\uparrow)}}                                           \\
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Model}}   & \multicolumn{1}{c|}{\textbf{Method}}    & \multicolumn{1}{c}{\textbf{Greedy}} & \multicolumn{1}{c}{\textbf{Beam}} & \multicolumn{1}{c}{\textbf{Greedy}} & \multicolumn{1}{c}{\textbf{Beam}} & \multicolumn{1}{c}{\textbf{Greedy}} & \multicolumn{1}{c}{\textbf{Beam}} & \multicolumn{1}{c}{\textbf{Greedy}} & \multicolumn{1}{c}{\textbf{Beam}} & \multicolumn{1}{c}{\textbf{Greedy}} & \multicolumn{1}{c}{\textbf{Beam}} \\
\arrayrulecolor{black}
\hline\hline
 \multirow{8}{*}{\rotatebox{90}{TL;DR}} & \multirow{4}{*}{GPT-J-6B}   & SFT  & 83.54  & 89.21 &   53.48   &   64.18  & -1.63  & -1.25   &  90.30  &  91.53  &   26.01    &  26.74  \\
 \cline{3-13}
 &
   & PPO & 75.88   &  83.10  &  47.52  &  54.40  &  -1.80     & -1.35 &  89.78  &  91.32   &   23.28  &  23.55 \\ &

& DPO &   82.55  &  88.12  &   54.09  &  61.70 &  -1.65   &  -1.33   &   90.22  &  91.27   &  26.28 &  \textbf{27.24}  \\
\arrayrulecolor{black}\cline{3-13}
& & MPO    &   \textbf{86.82}  &  \textbf{91.61}   &  \textbf{59.39}  & \textbf{72.10}  & \textbf{-1.41}  &  \textbf{-1.10}  &  \textbf{91.20}   &   \textbf{92.20}  &  \textbf{26.49}  &  26.10  \\
\arrayrulecolor{black}\cline{2-13}                        
& \multirow{2}{*}{Mistral-7B} & SFT  &  82.74  &   87.85  &    24.72   &   41.87    &  -1.81  &   -1.48  & 90.04 &  90.96  &  \textbf{25.02}  &  \textbf{25.32} \\
\arrayrulecolor{black}\cline{3-13}
% \midrule
& & MPO    &  \textbf{89.39}   &   \textbf{92.12}  &   \textbf{49.56} &   \textbf{61.90}   &   \textbf{-1.37}  &  \textbf{-1.25}  &  \textbf{91.53}  &   \textbf{91.82} & 25.01  & 24.85  \\
\arrayrulecolor{black}\cline{2-13}                        
& \multirow{2}{*}{LLaMA2-7B} & SFT    &  77.68  &  84.92   &    \textbf{23.36}   &   29.06   & -2.05   & -1.65 & 89.56 &  90.58 &  \textbf{23.33}  &  \textbf{24.31}  \\
\arrayrulecolor{black}\cline{3-13}
& & MPO     &   \textbf{78.03}  &  \textbf{85.33}   &  23.29  &   \textbf{29.39}   &  \textbf{-2.03}   &  \textbf{-1.64}  &  \textbf{89.65}  &  \textbf{90.67}  &  23.29 & 24.16 \\
\arrayrulecolor{black}
\hline
\multirow{4}{*}{\rotatebox{90}{XSUM}} & \multirow{2.5}{*}{Mistral-7B} & SFT  &  60.00  & 66.31   &   23.65   &     25.92  &  -1.97 &  -1.96   & 89.19 &  89.15  &  31.16  &  30.65   \\
\arrayrulecolor{black}\cline{3-13}
& & MPO    &   \textbf{64.57}  & \textbf{68.58}    & \textbf{24.33}  &   \textbf{27.18}  & \textbf{-1.90} &  \textbf{-1.85} &  \textbf{89.40} &  \textbf{89.53} &  \textbf{31.35} &  \textbf{31.11}  \\
 
\arrayrulecolor{black}\cline{2-13}            & \multirow{2}{*}{LLaMA2-7B} & SFT  &  57.57  &  65.80  &   24.40   &   27.50    & -2.06  &  -1.80   & 88.96 &  89.47  &  27.76  &  \textbf{30.36}   \\
\arrayrulecolor{black}\cline{3-13}
& & MPO    &  \textbf{60.48}   &   \textbf{67.31}  &  \textbf{26.50} &   \textbf{28.28}  & \textbf{-2.02}  & \textbf{-1.81}  & \textbf{89.10}  & \textbf{89.50} &  \textbf{28.36} & 30.32  \\
\arrayrulecolor{black}
% \arrayrulecolor{black}\bottomrule                   
\noalign{\hrule height 1pt}
\end{tabular}
}
\caption{\textbf{Comparison of MPO with SFT and human preference optimized models.} PPO (w/ human pref.) and DPO (w/ human pref.) represent models optimized with human preference data. Our method, MPO, utilizes results by beam search decoding from SFT model as chosen responses and temperature-scaled sampling generations from SFT model as rejected responses for preference optimization. The results indicate that the MPO enhances summarization outcomes in terms of faithfulness and relevance metrics compared to SFT and human preference optimized methods.
}
\end{table*}



==> tables/mint.tex <==
\begin{table}[t!]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{@{}c|c|cccc@{}}
\toprule 
\small\textbf{Method}& 
\small\textbf{Total}& \small\textbf{Non-empty}  & \small\textbf{Total tokens} & \small\textbf{$\text{Tokens}/\text{Non-empty}$} & \small{\textbf{Abstractiveness}} \\  
\midrule
\small{SFT} & \multirow{4}{*}{\small{6553}} & \small{5321} & \small{146806} & 
 \small{27.59}  &\small{0.323}  \\
\small{FAPO (Iter 1)} &  & \small{6548} & \small{191521}  & \small{35.99}   & \small{0.240} \\
\small{FAPO (Iter 2)} &  & \small{6549} & \small{184786}   & \small{34.73} & \small{0.176} \\
\small{FAPO (Iter 3)} &  & \small{6553} & \small{159751}   & \small{30.02} & \small{0.112} \\
\bottomrule
\end{tabular}
}
% \vspace{-0.5cm}
\caption{TL;DR (test), GPT, beam, Abstractiveness Score}
\label{table:mint}
\end{table}



% \begin{table}[tb!]
% \centering
% \resizebox{0.95\columnwidth}{!}{%
% \begin{tabular}{@{}c|ccc@{}}
% \toprule 
% \small\textbf{Method}& 
% \small\textbf{Mean}& \small\textbf{Median}  & \small\textbf{Variance} \\  
% \midrule
% \small{SFT} &  \small{0.727}  & \small{0.738} & \small{0.007}\\
% \small{FAPO (\textit{iteration 1})} &  \small{0.740}  & \small{0.748}   & \small{0.006} \\
% \small{FAPO (\textit{iteration 2})} &  \small{0.747}   & \small{0.754} & \small{0.006} \\
% \small{FAPO (\textit{iteration 3})} &  \small{0.057}   & \small{0.022} & \small{0.008} \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-0.5cm}
% \caption{TL;DR (test), GPT, beam, Abstractiveness Score}
% \label{table:mint}
% \end{table}

==> tables/mint_example_small.tex <==
\begin{table}[h!]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{p{2.1cm}p{12cm}}
\toprule
\small\textbf{Method} & \small\textbf{Text} \\ 
\midrule
\small{Prompt} & \small{SUBREDDIT: r/AskReddit TITLE: Any doctors or med students lurking? What is the process to become a doctor like? POST: I would like to become an anesthesiologist one day. I have thought about this a lot and would like to hear what it's like from some insiders. I am really not the type who can sit behind a desk all day. I'm prepared to sit at desks for studying, but I can't do it for 30+ years. I don't want to wear a suit and tie. I like to be up running around. Nothing else really interests me aside from extreme sports. I want to put my work in now and come out making a high salary. I don't want to climb the rungs of a corporate ladder. I've had friends with dads in construction, working 80+ hours a week. My dad as an engineer and programmer worked 80+ hours a week for years and his salary still isn't as high as an anesthesiologists (it's great for an engineer). I really just want to become an anesthesiologist.TL;DR:} \\

\small{SFT} & \small{I want to become an anesthesiologist. I'm not sure if I'm going about it the right way.}\\

\small{FAPO 1} & \small{I want to become an anesthesiologist. I want to know what it's like from an insider. What is the process like?} \\

\small{FAPO 2} & \small{I want to become an anesthesiologist. I want to know what it's like from an insider. What is the process to become a doctor like?} \\

\small{FAPO 3} & \small{Any doctors or med students lurking? What is the process to become a doctor like? I want to become an anesthesiologist one day.} \\

\bottomrule
\end{tabular}%
}
\caption{Examples for each iteration}
\end{table}

==> tables/plm.tex <==
\begin{table}[t]
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{c|c|c|ccc}
\noalign{\hrule height 1pt}
\small\textbf{Dataset}& \small\textbf{Model} & \small\textbf{Method} & \small\textbf{AlignScore $(\uparrow)$}  & \small\textbf{BARTScore $(\uparrow)$}  & \small\textbf{ROUGE-L $(\uparrow)$} \\
\hline
\hline
\multirow{9.5}{*}{\rotatebox{90}{TL;DR}} & \multirow{3}{*}{GPT-J}  & PLM    &   89.56 (79.06)    & -1.15 (-1.79)  &  19.28 (18.83)  \\
&& SFT    &   89.21 (83.54)   &   -1.25 (-1.63)    &   \textbf{26.74} (26.01)  \\
&& MPO   &  \textbf{91.61} (\textbf{86.82})      &  \textbf{-1.10} (\textbf{-1.41})    & 26.10 (\textbf{26.49})   \\
\cline{2-6}
& \multirow{3}{*}{Mistral} & PLM    &   83.23 (81.00)    & -1.46 (-1.77)  &  24.16 (24.25)  \\
&& SFT    &    87.85 (82.74)    & -1.48 (-1.81)  &  \textbf{25.32} (\textbf{25.02})  \\
&& MPO   &  \textbf{92.12} (\textbf{89.39}) &   \textbf{-1.25} (\textbf{-1.37})    &  24.85 (25.01)   \\
\cline{2-6}   
& \multirow{3}{*}{LLaMA2}   & PLM    &   84.99 (73.78)    & \textbf{-1.41} (-2.18)  &  21.81 (20.24)  \\
&& SFT    &   84.92 (77.68)   & -1.65 (-2.05)  &  \textbf{24.31} (\textbf{23.33})   \\
&& MPO   &  \textbf{85.33} (\textbf{78.03})       & -1.64 (\textbf{-2.03})     &  24.16 (23.29)  \\
\hline                      
\multirow{9.5}{*}{\rotatebox{90}{XSUM}} & \multirow{3}{*}{GPT-J}  & PLM    &   82.08 (58.92)    & -1.36 (-2.09)  &  11.90 (14.68)  \\
&& SFT    &   64.01 (52.66)   &   -1.59 (-1.97)    &   25.13 (24.41)  \\
&& MPO   &  65.26 (54.39)      & -1.58 (-1.95)    & 25.25 (24.72)   \\
\cline{2-6}
& \multirow{3}{*}{Mistral}  & PLM    &   76.65 (52.71)    & -1.54 (-2.83)  &  13.97 (14.73)  \\
&& SFT    &   66.31 (60.00)   &   -1.96 (-1.97)    &   30.65 (31.16)  \\
&& MPO   &  68.58 (64.57)      &  -1.85 (-1.90)    &  31.11 (31.35)   \\
\cline{2-6}
& \multirow{3}{*}{LLaMA2}   & PLM    &   73.57 (50.80)    & -1.99 (-3.28)  &  12.61 (13.25)  \\
&& SFT    &   65.80 (57.57)  &   -1.80 (-2.06)    &  30.36 (27.76) \\
&& MPO   &  67.31 (60.48)       &  -1.81 (-2.02)    &  30.32 (28.36)  \\
\noalign{\hrule height 1pt}
\end{tabular}
}
\caption{\textbf{Comparison of MPO with SFT}. MPO demonstrates generally robust results across various language models (Mistral and LLaMA2) on both the TL;DR and XSUM datasets. The results are based on a beam search decoding strategy, while the results in parentheses are based on a greedy decoding strategy.}
\label{table:models}
\end{table}

==> tables/significant_tests.tex <==
\begin{table}[t!]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{c|c|c|l|c|c}
\toprule
\textbf{Dataset} &\textbf{Comparison} & \textbf{Model} &\textbf{Metric} & \textbf{T-statistic} & \textbf{P-value} \\ \hline \hline

 \multirow{24}{*}{\rotatebox{90}{TL;DR}} & \multirow{12}{*}{SFT vs MPO}

& \multirow{5}{*}{GPT-J}& AlignScore & -11.1680 & 7.8936e-29 \\
                            &&& FactCC     & -6.1141  & 9.9881e-10 \\ 
                            &&& BARTScore  & -24.5166 & 8.1709e-130 \\
                            &&& BS-Fact    & -25.8462 & 1.0534e-143 \\
                            &&& Rouge-L    & -1.08255 & 0.2790 \\
                            
                            \cline{3-6}

&& \multirow{4}{*}{Mistral}& AlignScore & {} & {} \\
                            &&& FactCC     & {}  & {} \\ 
                            &&& BARTScore  & {} & {} \\
                            &&& BS-Fact    & {} & {} \\ \cline{3-6}
                            
&& \multirow{4}{*}{LLaMA2}& AlignScore & {} & {} \\
                            &&& FactCC     & {}  & {} \\ 
                            &&& BARTScore  & {} & {} \\
                            &&& BS-Fact    & {} & {} \\ \cline{2-6}
 
{}& \multirow{12}{*}{DPO vs MPO}

& \multirow{5}{*}{GPT-J}& AlignScore & -8.6351 & 6.5466e-18  \\
                            &&& FactCC     & -6.7249  & 1.8310e-11 \\ 
                            &&& BARTScore  & -21.3480 & 2.0353e-99 \\
                            &&& BS-Fact    & -21.3883 & 8.8545e-100 \\
                            &&& Rouge-L    & -2.2391 & 0.0252\\
                            
                            \cline{3-6}

&& \multirow{4}{*}{Mistral}& AlignScore & {} & {} \\
                            &&& FactCC     & {}  & {} \\ 
                            &&& BARTScore  & {} & {} \\
                            &&& BS-Fact    & {} & {} \\ \cline{3-6}
                            
&& \multirow{4}{*}{LLaMA2}& AlignScore & {} & {} \\
                            &&& FactCC     & {}  & {} \\ 
                            &&& BARTScore  & {} & {} \\
                            &&& BS-Fact    & {} & {} \\ \cline{3-6}



\bottomrule
\end{tabular}
}
\caption{Statistical comparison between DPO and MPO across various metrics.}
\label{table:signincant_tests}
\end{table}




==> tables/temperature.tex <==
\begin{table*}[t]
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{c|c|c|ccccc}
\noalign{\hrule height 1pt}
\small\textbf{Dataset}& \small\textbf{Model} & \small\textbf{Method} & \small\textbf{AlignScore $(\uparrow)$} & \small\textbf{FactCC $(\uparrow)$} & \small\textbf{BARTScore $(\uparrow)$}  & \small\textbf{BS-Fact $(\uparrow)$} & \small\textbf{ROUGE-L $(\uparrow)$} \\
\hline
\hline
\multirow{9.5}{*}{\rotatebox{90}{TL;DR}} & \multirow{3}{*}{GPT-J} & Beam search      &   \textbf{89.19}    &  \textbf{64.00} & \textbf{-1.24} & \textbf{91.56} & \textbf{27.00}   \\
&& Sampling (temp1)   &   57.68     &  32.27    &  -2.94 & 87.43 & 19.34  \\
&& Sampling (temp5) & 24.66  &  3.00     &   -6.89 & 80.57 & 8.73  \\
\cline{2-8}   
& \multirow{3}{*}{Mistral}   & Beam search     &  \textbf{87.47}   & \textbf{42.21}  & \textbf{-1.46} & \textbf{91.00} & \textbf{25.18}   \\
&& Sampling (temp1)   &    58.70    &  17.84    & -3.14  & 87.30 & 18.43 \\
&& Sampling (temp5)   &   22.96     &   3.45   & -7.14 & 79.74 & 8.35   \\
\cline{2-8}   
& \multirow{3}{*}{LLaMA2}   & Beam search     &   \textbf{84.72}  & \textbf{29.63}  & \textbf{-1.65} & \textbf{90.54} & \textbf{24.41}    \\
&& Sampling (temp1)   &    64.23    &  20.47    &  -2.71 & 88.12 & 19.69  \\
&& Sampling (temp5)   &  23.27  &  2.33    &  -7.12 & 79.82 & 8.51  \\
\hline                      
\multirow{9.5}{*}{\rotatebox{90}{XSUM}} & \multirow{3}{*}{GPT-J} & Beam search    &  \textbf{64.55}   &   \textbf{29.28}    &  \textbf{-1.59} &  \textbf{89.95} &  \textbf{25.34} \\
&& Sampling (temp1)   &    28.12    &  20.88    &  -2.99 & 86.95 & 17.77  \\
&& Sampling (temp5)   &  14.33  &   1.86    &   -6.91 &  80.01 & 6.95 \\
\cline{2-8}
& \multirow{3}{*}{Mistral}   & Beam search    &  \textbf{66.76}   &   \textbf{25.49}   & \textbf{-1.96} & \textbf{89.17} & \textbf{30.57}  \\
&& Sampling (temp1)   &     43.48   &   18.25  &  -2.81 & 87.50 & 22.81  \\
&& Sampling (temp5)   &    20.07  &  4.19   &  -7.41 & 78.52 & 6.82  \\
\cline{2-8}   
& \multirow{3}{*}{LLaMA2}   & Beam search     &  \textbf{66.57}   & \textbf{26.88}  &  \textbf{-1.81} & \textbf{89.50} & \textbf{30.48}   \\
&& Sampling (temp1)   &   47.65    &   21.69   &  -2.49 & 88.10 & 23.76  \\
&& Sampling (temp5)   &    17.65    &   3.08   &  -7.41 & 78.82 & 7.39  \\
\noalign{\hrule height 1pt}
\end{tabular}
}
\caption{\textbf{Results of Evaluation Metrics for Chosen and Rejected Samples}. Summaries generated with beam search outperformed those from temperature sampling across all metrics. For GPT-J, summaries generated with beam search were used as the chosen samples, while those from temperature-5 sampling were the rejected samples. Similarly, for Mistral and LLaMA2, summaries generated with beam search were chosen, while those from temperature-1 sampling were rejected.}
\label{table:temperature}
\end{table*}
